Token Composition: A Graph Based on EVM Logs

Tokens have proliferated across blockchains in terms of number, market capitalisation, and utility. Some tokens are tokenised versions of existing tokens, known variously as wrapped tokens, fractional tokens or shares. The repeated application of this process creates tokens with arbitrarily many layers of composition. We perform an empirical analysis of token composition on the Ethereum blockchain. We introduce a graph that represents the tokenisation of tokens by other tokens, and we show that the graph contains non-trivial topological structure. We relate properties of the graph, for example, connected components and cyclic structure, to the tokenisation process. For example, we identify the longest directed path and its corresponding sequence of tokens, and we visualise the connected components relating to a stablecoin and a non-fungible token protocol. Our goal is to explore and visualise what has been built with tokens, rather than propose new constructions.

==> acronyms.tex <==
\newacronym{dao}{DAO}{Decentralised Autonomous Organisation}
\newacronym{dex}{DEX}{decentralised exchange}
\newacronym{evm}{EVM}{Ethereum Virtual Machine}
\newacronym{nft}{NFT}{non-fungible token}
\newacronym{roi}{RoI}{Republic of Ireland}
\newacronym{rpc}{RPC}{remote procedure call}
\newacronym{setu}{SETU}{South East Technological University}

